Probing Quantum Phenomena through Photoproduction in Relativistic Heavy-Ion Collisions

Photoproduction in ultra-peripheral relativistic heavy-ion collisions displays many unique features, often involving quantum mechanical coherence and two-source interference between photon emission from the two ions. We review the recent experimental results from RHIC and the LHC and theoretical studies of coherent vector meson photoproduction, emphasizing the quantum mechanical aspects of the interactions and the entanglement between the final state particles. These studies enrich our understanding of non-local realism, underscore the critical role of the polarization of the photon source, quantum interference and nuclear effect on the gluon distribution. It paves a way for quantitatively probing the quantum nature of these high-energy nuclear collisions.

==> Section4-2.tex <==
\hspace{2em}One of the first manifestations of coherence in photoproduction comes about when considering a single nucleus as a target: the amplitudes for interactions on individual nucleons can add in-phase:
\begin{equation}
    \sigma= \Sigma_i A_i e^{(i\vec{k}\cdot \vec{R}_i)}    \label{eq:onenucleoncoherence}
\end{equation}
where the sum $i$ runs over the nucleons in the target, $A_i$ is the amplitude to scatter from nucleon $i$ at position $\vec{R}_i$ and $\vec{k}$ is the momentum transfer from the target.  When $|\vec{k}|<\hbar/R_A$, the exponential is near one for all nucleons, and the cross-section goes as the square of the number of nucleons.  For large $\vec{k}$, the phase is random and the cross section scales as the number of nucleons. Equation \ref{eq:onenucleoncoherence} neglects a few factors.  The first is that if a photon enters the nucleus in a $q\overline q$ state, then it may interact multiple times as it traverses the nucleus, altering the coherent relation above.  This can be accounted for with a Glauber calculation, discussed in the next section. 



{\bf the following belongs elsewhere}

 
